High-Impact Innovations and Hidden Gender Disparities in Inventor-Evaluator Networks

We study of millions of scientific, technological, and artistic innovations and find that the innovation gap faced by women is far from universal. No gap exists for conventional innovations. Rather, the gap is pervasively rooted in innovations that combine ideas in unexpected ways - innovations most critical to scientific breakthroughs. Further, at the USPTO we find that female examiners reject up to 33 percent more unconventional innovations by women inventors than do male examiners, suggesting that gender discrimination weakly explains this innovation gap. Instead, new data indicate that a configuration of institutional practices explains the innovation gap. These practices compromise the expertise women examiners need to accurately assess unconventional innovations and then "over-assign" women examiners to women innovators, undermining women's innovations. These institutional impediments negatively impact innovation rates in science but have the virtue of being more amenable to actionable policy changes than does culturally ingrained gender discrimination.

==> absoluteClaimsReg.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
            DV = $\Delta{Absolute}$          &\multicolumn{1}{c}{(USA Granted Patents)}         \\
\midrule
           &                     \\
Proportion Female Inventors           &       0.319\sym{***}\\
                    &    (0.0380 )         \\
\addlinespace
Atypicality             &    0.00797\sym{***}\\
                    & (0.0000737)         \\
\addlinespace
Year FE          &     Y \\
\addlinespace
Team Size FE          &     Y \\
\addlinespace
CPC Code FE          &     Y \\
\addlinespace
\midrule
Observations        &      241878         \\
\(R^{2}\)    &       0.0319         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> allAtypicalMeasuresTogether.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{1}{c}{Min} &\multicolumn{1}{c}{Mean} &\multicolumn{1}{c}{Median} &\multicolumn{1}{c}{Empirical} \\
                    
\midrule
Patent Acceptance               &       && &              \\
Proportion Female Inventors &  -0.272\sym{***} & -0.278\sym{***} & -0.273\sym{***} & -0.267\sym{***}\\
                    &    (0.0174)  &    (0.02011)  &    (0.0197)  &    (0.0195)       \\
\addlinespace

Atypicality             &     0.0001534\sym{***} & 0.0001683\sym{***} &     0.0001984\sym{***} &-0.1463\\
                    & (0.0000397)         \\
\addlinespace
Proportion Female Inventors $\times$ Atypicality&   -0.0005019\sym{***}\\
                    &  (0.000012)         \\
\addlinespace

Big Entity             &    0.590\sym{***}\\
                    & (0.00806)         \\
\addlinespace

\addlinespace
Female Examiner            &      -0.102\sym{***}\\
                    & (0.00793)         \\
\addlinespace

\addlinespace
Average Inventor Experience           &     -0.00111\sym{***}\\
                    & (0.0000527)         \\
\addlinespace

\addlinespace
Average Examiner Experience           &     0.00118\sym{***}\\
                    & (0.0000129)         \\
\addlinespace


\midrule
Observations        &      392622         \\
Pseudo \(R^{2}\)    &        0.0915         \\


% Patent Acceptance    & & &   \\
% Proportion Female Inventors           &       -0.278\sym{***} & & &\\
%                     &    (0.02011)      & & &   \\
% \addlinespace

% Atypicality             &     0.0001683\sym{***}  & & & \\
%                     & (0.0000302)        & & &   \\
% \addlinespace
% Proportion Female Inventors $\times$ Atypicality&   -0.0002626\sym{**}  & & & \\
%                     &  (0.0000868)      & & &     \\
% \addlinespace

% Big Entity             &    0.590\sym{***}  & & & \\
%                     & (0.00806)      & & &     \\
% \addlinespace

% \addlinespace
% Female Examiner            &      -0.101\sym{***}  & & & \\
%                     & (0.00793)      & & &     \\
% \addlinespace

% \addlinespace
% Average Inventor Experience           &     -0.00111\sym{***}  & & & \\
%                     & (0.0000527)   & & &        \\
% \addlinespace

% \addlinespace
% Average Examiner Experience           &     0.00118\sym{***}  & & & \\
%                     & (0.0000129)      & & &     \\
% \addlinespace


% \midrule
% Observations        &      392622     & & &      \\
% Pseudo \(R^{2}\)    &        0.0915      & & &     \\

% \midrule
% Patent Acceptance              &                     &                     &         &            \\
% Proportion Female Inventors           &      -0.531\sym{***}&      -1.011\sym{***}&      -0.769\sym{***} & \\
%                     &    (0.0145)         &    (0.0291)         &    (0.0259)     &     \\
% \addlinespace
% Atypicality             &    0.000493\sym{***}&                     &            &         \\
%                     & (0.0000317)         &                     &           &          \\
% \addlinespace
% Proportion Female Inventors $\times$ Atypicality&   -0.000829\sym{***}&                     &           &          \\
%                     &  (0.000107)         &                     &          &           \\
% \midrule
% Observations        &      511938         &      198739         &      209249     &    \\
% Pseudo \(R^{2}\)    &       0.042         &       0.046         &       0.034     &    \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> allAtypicalTabularx.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabularx}{\linewidth}{ p{\dimexpr.29\linewidth-2\tabcolsep-1.3333\arrayrulewidth} X X X X }  
\toprule
% \hline
& Min & Mean & Median & Empirical\\
                    % &\multicolumn{1}{c}{Min} &\multicolumn{1}{c}{Mean} &\multicolumn{1}{c}{Median} &\multicolumn{1}{c}{Empirical} \\
                    
\midrule
Patent Acceptance               &       & & &              \\
% \hline
Proportion Female \\Inventors &  -0.272\sym{***} & -0.278\sym{***} & -0.273\sym{***} & -0.267\sym{***}\\
                    &    (0.0174)  &    (0.02011)  &    (0.0197)  &    (0.0195)       \\
\addlinespace

Atypicality             &     0.0001534\sym{***} & 0.0001683\sym{***} &     0.0001984\sym{***} &-0.1463\\
                    & (0.0000397)    & (0.0000302)   & (0.0000296)     & (0.0770)        \\
\addlinespace
Proportion Female \\Inventors $\times$ Atypicality&   -0.0005019\sym{***} & -0.0002626\sym{**} & -0.0002396\sym{**} &-0.520\sym{*}\\
                    &  (0.000012)   &  (0.0000868)   &  (0.0000864)  &  (0.248)        \\
\addlinespace

Big Entity             &    0.590\sym{***} &    0.590\sym{***}  &    0.590\sym{***} &    0.588\sym{***}\\
                    & (0.00806)    & (0.00806)   & (0.00806)  & (0.00807)        \\
\addlinespace

\addlinespace
Female Examiner            &      -0.102\sym{***} &      -0.101\sym{***} &      -0.101\sym{***}&      -0.102\sym{***}\\
                    & (0.00793)    & (0.00793)   & (0.00793)     & (0.00793)      \\
\addlinespace

\addlinespace
Average Inventor \\Experience           &     -0.00111\sym{***} &     -0.00111\sym{***}  &     -0.00110\sym{***} &     -0.00112\sym{***}\\
                    & (0.0000527)    & (0.0000527)   & (0.0000528)   & (0.0000528)       \\
\addlinespace

\addlinespace
Average Examiner \\Experience           &     0.00118\sym{***}  &     0.00118\sym{***} &     0.00118\sym{***}&     0.00117\sym{***}\\
                    & (0.0000129)   & (0.0000129) & (0.0000129)  & (0.0000128)      \\
\addlinespace


\midrule
Observations        &      392622     & 392622 & 392622 & 392606    \\
Pseudo \(R^{2}\)    &        0.0915 &        0.0915 &        0.0916 &        0.0915         \\


% Patent Acceptance    & & &   \\
% Proportion Female Inventors           &       -0.278\sym{***} & & &\\
%                     &    (0.02011)      & & &   \\
% \addlinespace

% Atypicality             &     0.0001683\sym{***}  & & & \\
%                     & (0.0000302)        & & &   \\
% \addlinespace
% Proportion Female Inventors $\times$ Atypicality&   -0.0002626\sym{**}  & & & \\
%                     &  (0.0000868)      & & &     \\
% \addlinespace

% Big Entity             &    0.590\sym{***}  & & & \\
%                     & (0.00806)      & & &     \\
% \addlinespace

% \addlinespace
% Female Examiner            &      -0.101\sym{***}  & & & \\
%                     & (0.00793)      & & &     \\
% \addlinespace

% \addlinespace
% Average Inventor Experience           &     -0.00111\sym{***}  & & & \\
%                     & (0.0000527)   & & &        \\
% \addlinespace

% \addlinespace
% Average Examiner Experience           &     0.00118\sym{***}  & & & \\
%                     & (0.0000129)      & & &     \\
% \addlinespace


% \midrule
% Observations        &      392622     & & &      \\
% Pseudo \(R^{2}\)    &        0.0915      & & &     \\

% \midrule
% Patent Acceptance              &                     &                     &         &            \\
% Proportion Female Inventors           &      -0.531\sym{***}&      -1.011\sym{***}&      -0.769\sym{***} & \\
%                     &    (0.0145)         &    (0.0291)         &    (0.0259)     &     \\
% \addlinespace
% Atypicality             &    0.000493\sym{***}&                     &            &         \\
%                     & (0.0000317)         &                     &           &          \\
% \addlinespace
% Proportion Female Inventors $\times$ Atypicality&   -0.000829\sym{***}&                     &           &          \\
%                     &  (0.000107)         &                     &          &           \\
% \midrule
% Observations        &      511938         &      198739         &      209249     &    \\
% Pseudo \(R^{2}\)    &       0.042         &       0.046         &       0.034     &    \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabularx}
}


==> atypicalEmpirical.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
% \toprule
                    &\multicolumn{1}{c}{(US Patent Applications)}         \\
\midrule
Patent Acceptance               &                     \\
Proportion Female Inventors           &       -0.267\sym{***}\\
                    &    (0.0195)         \\
\addlinespace

Atypicality (Empirical)             &     -0.1463\\
                    & (0.0770)         \\
\addlinespace
Proportion Female Inventors $\times$ Atypicality (Empirical)&   -0.520\sym{*}\\
                    &  (0.248)         \\
\addlinespace

Big Entity             &    0.588\sym{***}\\
                    & (0.00807)         \\
\addlinespace

\addlinespace
Female Examiner            &      -0.102\sym{***}\\
                    & (0.00793)         \\
\addlinespace

\addlinespace
Average Inventor Experience           &     -0.00112\sym{***}\\
                    & (0.0000528)         \\
\addlinespace

\addlinespace
Average Examiner Experience           &     0.00117\sym{***}\\
                    & (0.0000128)         \\
\addlinespace


\midrule
Observations        &      392606         \\
Pseudo \(R^{2}\)    &        0.0915         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize The base case for big entity is small entity.}\\
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> atypicalMeanReg.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
% \toprule
                    &\multicolumn{1}{c}{(US Patent Applications)}         \\
\midrule
Patent Acceptance               &                     \\
Proportion Female Inventors           &       -0.278\sym{***}\\
                    &    (0.02011)         \\
\addlinespace

Atypicality (Mean)             &     0.0001683\sym{***}\\
                    & (0.0000302)         \\
\addlinespace
Proportion Female Inventors $\times$ Atypicality (Mean)&   -0.0002626\sym{**}\\
                    &  (0.0000868)         \\
\addlinespace

Big Entity             &    0.590\sym{***}\\
                    & (0.00806)         \\
\addlinespace

\addlinespace
Female Examiner            &      -0.101\sym{***}\\
                    & (0.00793)         \\
\addlinespace

\addlinespace
Average Inventor Experience           &     -0.00111\sym{***}\\
                    & (0.0000527)         \\
\addlinespace

\addlinespace
Average Examiner Experience           &     0.00118\sym{***}\\
                    & (0.0000129)         \\
\addlinespace


\midrule
Observations        &      392622         \\
Pseudo \(R^{2}\)    &        0.0915         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize The base case for big entity is small entity.}\\
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> atypicalMedian.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
% \toprule
                    &\multicolumn{1}{c}{(US Patent Applications)}         \\
\midrule
Patent Acceptance               &                     \\
Proportion Female Inventors           &       -0.273\sym{***}\\
                    &    (0.0197)         \\
\addlinespace

Atypicality (Median)             &     0.0001984\sym{***}\\
                    & (0.0000296)         \\
\addlinespace
Proportion Female Inventors $\times$ Atypicality (Median)&   -0.0002396\sym{**}\\
                    &  (0.0000864)         \\
\addlinespace

Big Entity             &    0.590\sym{***}\\
                    & (0.00806)         \\
\addlinespace

\addlinespace
Female Examiner            &      -0.101\sym{***}\\
                    & (0.00793)         \\
\addlinespace

\addlinespace
Average Inventor Experience           &     -0.00110\sym{***}\\
                    & (0.0000528)         \\
\addlinespace

\addlinespace
Average Examiner Experience           &     0.00118\sym{***}\\
                    & (0.0000129)         \\
\addlinespace


\midrule
Observations        &      392622         \\
Pseudo \(R^{2}\)    &        0.0916         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize The base case for big entity is small entity.}\\
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> atypicalRateTable.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{1}{c}{USA}         &\multicolumn{1}{c}{UK}         &\multicolumn{1}{c}{Canada}         \\
\midrule

Male Only Inventor Team   &   0.668&      0.651&      0.870\\
\addlinespace
Female Only Inventor Team   &   0.558&      0.540&      0.850\\
\addlinespace
\midrule

Male Majority   &   0.658&      0.661&      0.852\\
\addlinespace
Female Majority   &   0.578&      0.608&      0.849\\
\addlinespace

% \bottomrule

\end{tabular}
}


==> deltaIndepInteractReg.tex <==
% {
% \def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
% \begin{tabular}{l*{1}{c}}
% \toprule
%             DV = $\Delta{Absolute}$           &\multicolumn{1}{c}{(USA Granted Patents)}         \\
% \midrule
%           &                     \\
% Proportion Female Inventors           &        0.211\sym{***}\\
%                     &    (0.0418)         \\
% \addlinespace
% Boundary-Pushing              &    0.000998\sym{***}\\
%                     & (0.0000861)         \\
% \addlinespace
% Proportion Female Inventors $\times$ Boundary-Pushing              &    -0.00109\sym{***}\\
%                     & (0.000264)         \\
% \addlinespace
% Big Entity             &    -0.4668202\sym{***}\\
%                     & (0.00806)         \\
% \addlinespace

% \addlinespace
% Female Examiner            &      -0.102\sym{***}\\
%                     & (0.00793)         \\
% \addlinespace

% \addlinespace
% Average Inventor Experience           &     -0.00111\sym{***}\\
%                     & (0.0000527)         \\
% \addlinespace

% \addlinespace
% Average Examiner Experience           &     0.00118\sym{***}\\
%                     & (0.0000129)         \\
% \addlinespace


% Year FE          &     Y \\
% \addlinespace
% Team Size FE          &     Y \\
% \addlinespace
% CPC Code FE          &     Y \\
% \addlinespace
% \midrule
% Observations        &      241875         \\
% \(R^{2}\)    &       0.3887         \\
% \bottomrule
% \multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
% \multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
% \end{tabular}
% }


==> iterativeOld.tex <==
% \documentclass{article}
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{geometry}
% \geometry{margin=1in}

% \begin{document}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\small
\renewcommand{\arraystretch}{0.8}

\begin{tabularx}{\linewidth}{ p{\dimexpr.15\linewidth-2\tabcolsep-1.3333\arrayrulewidth} X X X X X X X}
% \begin{tabularx}{\linewidth}{p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}
%                                   p{\dimexpr.15\linewidth-2\tabcolsep}}
\toprule
% DV =\\Patent \\Acceptance &  Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6  \\
DV = Patent Acceptance &  Controls Only & With Examiner Features & With Inventor Features (no gender) & With Inventor Gender Feature & With Atypicality & With Gender $\times$ Atypicality \\
% Model 1: Controls Only, Model 2: With Examiner Features, Model 3: With Inventor Features (no gender), Model 4: With Inventor Gender Feature, Model 5: With Atypicality, Model 6: With Gender Atypicality Interaction

\midrule
Proportion \\Female \\Inventors &  --- & --- &  --- & --- &--- & -0.270\sym{***} \\
                            &        &    & & &     &    (1.79e-2)   \\
\addlinespace
Atypicality &     --- & --- &     --- & --- &--- &1.50e-4\sym{***} \\
            &              &         &&&   & (3.82e-5)           \\
\addlinespace
Proportion \\Female \\Inventors $\times$ \\Atypicality &   --- & ---  &  --- & --- &--- & -3.73e-4\sym{***} \\
                           &           &&&     &             &  (1.11e-4)                \\
\addlinespace
Big Entity &    ---&  --- & --- &--- &     0.592\sym{***}  &     0.590\sym{***} \\
           &              &    &&&  (8.05e-3)    & (8.06e-3)             \\
\addlinespace
Female Examiner &   ---    &  --- & --- &---&     -0.1040\sym{***} &      -0.101\sym{***}\\
                 &           &    &&& (7.92e-3)     & (7.93e-3)                    \\
\addlinespace
Average Inventor \\Experience &     --- &  --- & --- &---&   -1.11e-3\sym{***}  &     -1.11e-3\sym{***} \\
                            &          &&&    &   (5.26e-5) & (5.28e-5)        \\
\addlinespace
Average \\Examiner \\Experience &     --- &  --- & --- &--- &    1.18e-3\sym{***}  &     1.18e-3\sym{***}\\
                            &            &&&        &      (1.28e-3)     & (1.29e-5)                       \\
\addlinespace
Year FE &     Y  &     Y &    Y &    Y &    Y &    Y\\
\addlinespace
Team \\Size FE &     Y  &     Y &    Y & Y &    Y &    Y\\\
\addlinespace
CPC \\Code FE &     Y  &     Y &    Y &  Y &    Y &    Y\\\
% \addlinespace
% \addlinespace
\midrule
% \addlinespace
Observations        &      393387      & 392791  & 392791 & 392791  & 392791 & 392791  \\
Pseudo \(R^{2}\)    &        0.0593 &        0.0910 &        0.0915   &        0.0910 &        0.0915   &        0.0910     \\
AIC    &        469737.9 &        452772.6  &        0.0915    &        0.0910 &        0.0915    &        0.0910    \\
BIC   &         471315.9 &        454393.9 &        0.0915    &        0.0910 &        0.0915 &        0.0910      \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\

\end{tabularx}


==> iterativeRegOnly2Models.tex <==
% \documentclass{article}
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{geometry}
% \geometry{margin=1in}

% \begin{document}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\small
\renewcommand{\arraystretch}{0.8}

\begin{tabularx}{\linewidth}{ p{\dimexpr.4\linewidth-2\tabcolsep-1.3333\arrayrulewidth} X X X}

\toprule
DV = Patent Acceptance &  Baseline Model & Full Model \\
\midrule
Proportion \\Female \\Inventors &  ---  & -0.270\sym{***} \\
                            &            &  (1.79e-2)   \\
\addlinespace
Atypicality &     --- &  1.50e-4\sym{***} \\
            &                  & (3.82e-5)           \\
\addlinespace
Proportion \\Female \\Inventors $\times$ \\Atypicality &   --- & -3.73e-4\sym{***} \\
                           &                     &  (1.11e-4)                \\
\addlinespace
Big Entity &    0.592\sym{***} &     0.590\sym{***} \\
           &        (8.05e-3)     & (8.06e-3)             \\
\addlinespace
Female\\Examiner &   -0.104\sym{***}   & -0.101\sym{***}\\
                 &       (7.92e-3)     & (7.93e-3)                    \\
\addlinespace
Average \\Inventor \\Experience &     -1.11e-3\sym{***} &   -1.11e-3\sym{***} \\
                            &    (5.26e-5)      & (5.28e-5)        \\
\addlinespace
Average \\Examiner \\Experience &      1.18e-3\sym{***} &  1.18e-3\sym{***}\\
                            &       (1.28e-5)     & (1.29e-5)                       \\
\addlinespace
Year FE &     Y  &     Y \\
\addlinespace
Team \\Size FE &     Y  &     Y\\
\addlinespace
CPC \\Code FE &     Y  &     Y \\
\midrule
% \addlinespace
Observations        &      392791     & 392791  \\
Pseudo \(R^{2}\)    &        0.0910 & 0.0915    \\
AIC    &     452772.6   &        452530.4    \\
BIC   &       454393.9  &      454184.3      \\
\bottomrule
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabularx}


==> mainRegression.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
% \toprule
                    &\multicolumn{1}{c}{(US Patent Applications)}         \\
\midrule
Patent Acceptance               &                     \\
Proportion Female Inventors           &       -0.272\sym{***}\\
                    &    (0.0174)         \\
\addlinespace

Atypicality             &     0.0001534\sym{***}\\
                    & (0.0000397)         \\
\addlinespace
Proportion Female Inventors $\times$ Atypicality&   -0.0005019\sym{***}\\
                    &  (0.000012)         \\
\addlinespace

Big Entity             &    0.590\sym{***}\\
                    & (0.00806)         \\
\addlinespace

\addlinespace
Female Examiner            &      -0.102\sym{***}\\
                    & (0.00793)         \\
\addlinespace

\addlinespace
Average Inventor Experience           &     -0.00111\sym{***}\\
                    & (0.0000527)         \\
\addlinespace

\addlinespace
Average Examiner Experience           &     0.00118\sym{***}\\
                    & (0.0000129)         \\
\addlinespace


\midrule
Observations        &      392622         \\
Pseudo \(R^{2}\)    &        0.0915         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize The base case for big entity is small entity.}\\
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> maintenanceFee.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
                    &\multicolumn{1}{c}{(USA)}         \\
\midrule
DV = Any Maintenance Fee Paid (Indicator)               &                     \\
Proportion Female Inventors           &      -0.1744\sym{***}\\
                    &    (0.0221)         \\
\addlinespace
Atypicality             &    0.0004415\sym{***}\\
                    & (0.0000456)         \\
\addlinespace
Entity &   0.0277572\sym{*}\\
                    &  (0.0110)         \\
\midrule
Observations        &       263372         \\
Pseudo \(R^{2}\)    &       0.1847         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\multicolumn{2}{l}{\footnotesize Year, Team Size, and CPC Code Fixed Effects}\\
\end{tabular}
}


==> mergedClaimsRegResults.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
            DV        &\multicolumn{1}{c}{$\Delta{Absolute}$}   &\multicolumn{1}{c}{$\Delta{Relative}$}   &\multicolumn{1}{c}{$n_{grant}$}         \\
\midrule
           &                     \\
Proportion Female Inventors           &       0.319\sym{***} & 0.0650\sym{***} & -0.112\sym{***}\\
                    &    (0.0380)    & (1.07e-2) & (2.30e-2)   \\
\addlinespace
Boundary-Pushing             &    7.97e-3\sym{***} & 1.40e-4\sym{***}  & 3.47e-4\sym{***}  \\
                    & (7.37e-5)   & (2.07e-5) & (4.46e-5)       \\
\addlinespace
Year FE          &     Y & Y & Y \\
\addlinespace
Team Size FE          &     Y& Y & Y  \\
\addlinespace
CPC Code FE          &     Y& Y & Y\\
\addlinespace
\midrule
Observations        &      241878     & 241878 & 241878    \\
\(R^{2}\)    &       0.0319     & 0.0341 & 0.0887    \\
\bottomrule
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> numGrantReg.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
         DV = $n_{grant}$             &\multicolumn{1}{c}{(USA Granted Patents)}         \\
\midrule
           &                     \\
Proportion Female Inventors           &        -0.112\sym{***}\\
                    &    (0.0230)         \\
\addlinespace
Atypicality             &    0.000347 \sym{***}\\
                    & (0.0000446)         \\
\addlinespace
Year FE          &     Y \\
\addlinespace
Team Size FE          &     Y \\
\addlinespace
CPC Code FE          &     Y \\
\addlinespace
\midrule
Observations        &      241878         \\
\(R^{2}\)    &        0.0887         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> perceChangeIndepClaimsRegression.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
           DV = $\Delta{Relative}$           &\multicolumn{1}{c}{(USA Granted Patents)}         \\
\midrule
           &                     \\
Proportion Female Inventors           &       0.0650\sym{***}\\
                    &    (0.0107)         \\
\addlinespace
Atypicality             &    0.000140\sym{***}\\
                    & (0.0000207)         \\
\addlinespace
Year FE          &     Y \\
\addlinespace
Team Size FE          &     Y \\
\addlinespace
CPC Code FE          &     Y \\
\addlinespace
\midrule
Observations        &      241878         \\
\(R^{2}\)    &       0.0341         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> regAllCountries.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{D{.}{.}{-1}}}
\toprule
                    &\multicolumn{1}{c}{(All Countries)}         &\multicolumn{1}{c}{(UK)}         &\multicolumn{1}{c}{(Canada)}         \\
\midrule
Patent Acceptance              &                     &                     &                     \\
Proportion Female Inventors           &      -0.531\sym{***}&      -1.011\sym{***}&      -0.769\sym{***}\\
                    &    (0.0145)         &    (0.0291)         &    (0.0259)         \\
\addlinespace
Atypicality             &    0.000493\sym{***}&                     &                     \\
                    & (0.0000317)         &                     &                     \\
\addlinespace
Proportion Female Inventors $\times$ Atypicality&   -0.000829\sym{***}&                     &                     \\
                    &  (0.000107)         &                     &                     \\
\midrule
Observations        &      511938         &      198739         &      209249         \\
Pseudo \(R^{2}\)    &       0.042         &       0.046         &       0.034         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> regUkCanOnly.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
         DV = Patent Acceptance           &\multicolumn{1}{c}{(UK)}         &\multicolumn{1}{c}{(Canada)}         \\
\midrule
              &                     &                     \\
Proportion Female Inventors           &      -0.343\sym{***}&      -0.396\sym{***}\\
                    &    (0.0573)         &    (0.104)         \\
\addlinespace
Boundary-Pushing             &      0.00103\sym{***}&     0.000722\sym{*}\\
                    &  (0.000242)         &  (0.000280)         \\
\addlinespace
Year FE          &     Y&     Y  \\
\addlinespace
Team Size FE          &     Y &     Y \\

\midrule
Observations        &      28,715         &      15,611         \\
Pseudo \(R^{2}\)    &       0.0188         &       0.0556         \\
\bottomrule
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> regUkCanUSOnly.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(UK)}         &\multicolumn{1}{c}{(Canada)}         &\multicolumn{1}{c}{(USA)}         \\
\midrule
Patent Acceptance              &                     &                     &                     \\
Proportion Female Inventors           &      -0.265\sym{***}&      -0.447\sym{***}&      -0.267\sym{***}\\
                    &    (0.0407)         &    (0.0482)         &    (0.0148)         \\
\addlinespace
Atypicality             &      0.0102\sym{***}&     0.00594\sym{***}&  -0.0000976\sym{**} \\
                    &  (0.000281)         &  (0.000173)         & (0.0000314)         \\
\midrule
Observations        &      178424         &      170686         &      422535         \\
Pseudo \(R^{2}\)    &       0.227         &       0.189         &       0.062         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> timeDeltaRegression.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
            DV = ${T_{grant} - T_{filing}}$           &\multicolumn{1}{c}{(USA Granted Patents)}         \\
\midrule
          &                     \\
Proportion Female Inventors           &        33.0862\sym{***}\\
                    &    (4.740)         \\
\addlinespace
Boundary-Pushing              &    0.318\sym{***}\\
                    & (0.00920)         \\
\addlinespace
Year FE          &     Y \\
\addlinespace
Team Size FE          &     Y \\
\addlinespace
CPC Code FE          &     Y \\
\addlinespace
\midrule
Observations        &      241875         \\
\(R^{2}\)    &       0.3887         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}

